End-to-End Reinforcement Learning for Automatic Taxonomy Induction

We present a novel end-to-end reinforcement learning approach to automatic taxonomy induction from a set of terms. While prior methods treat the problem as a two-phase task (i.e., detecting hypernymy pairs followed by organizing these pairs into a tree-structured hierarchy), we argue that such two-phase methods may suffer from error propagation, and cannot effectively optimize metrics that capture the holistic structure of a taxonomy. In our approach, the representations of term pairs are learned using multiple sources of information and used to determine \textit{which} term to select and \textit{where} to place it on the taxonomy via a policy network. All components are trained in an end-to-end manner with cumulative rewards, measured by a holistic tree metric over the training taxonomies. Experiments on two public datasets of different domains show that our approach outperforms prior state-of-the-art taxonomy induction methods up to 19.6\% on ancestor F1.

==> 1-intro_v0.tex <==
%!TEX root = acl18-RL-tree.tex
% UTF-8 encoding

\section{Introduction}
%Taxonomies are of great importance to natural language processing as many tasks (question answering, short text understanding, etc.) benefit from the hypernymy relations discovered by these hierarchies.
Many tasks in natural language understanding (\eg, information extraction \cite{Demeester2016LiftedRI}, question answering \cite{Yang2017EfficientlyAT}, and textual entailment \cite{Sammons2012RecognizingTE}) rely on lexical \nop{semantic knowledge} resources in the form of term taxonomies (cf. rightmost column in Fig.~\ref{fig:toy}). 
Most existing taxonomies, such as WordNet \cite{miller1995wordnet} and Cyc \cite{lenat1995cyc} are manually curated, and thus may have limited coverage or be unavailable in some domains and languages. 
As a result, recent efforts have focused on automating the process of taxonomy induction.

% Existing taxonomies are generally constructed by human experts or in a crowd-sourcing manner.
% % For example, WordNet and Wikipedia are among the most popular manually constructed resources.
% However, it is both time-consuming and labor-intensive to construct taxonomies by the human for every language and domain.
% As a result, automatic taxonomy induction is always in great demand.
% Although there have been efforts on building taxonomies automatically, the problem is still far from solved due to multiple reasons. 
% The main reasons include but not limited to: 
% (1) The lack of standard benchmarks. Many evaluations are based on non-replicable experiments or require manual effort, which makes comparison and improvement based on previous works harder; 
% (2) The insufficiency of well defined evaluation metrics. Edge-based quality is certainly desired but global structure of a taxonomy is also important. Evaluation of a taxonomy is still an open question;
% (3) The complexity of the task itself and reasons above seem to make the res{}earch attention shift from building full-fledged taxonomies entirely or partly from scratch to the prior step of inducing hypernymy relations \cite{camacho2017we}.

% \todo{how to connect these two paragraphs.. is it good if we didn't fully address the problems above but mention them here?}
% Despite the challenges and difficulties of automating the process of taxonomy induction

% JS
As pointed out in \citet{gupta2017taxonomy,camacho2017we}, approaches towards automatic taxonomy induction are generally composed of two phases: 
(1) \textbf{hypernymy detection} (i.e., extracting term pairs that satisfy the ``is-a'' relation, such as (\mquote{panda},\mquote{mammal})) and 
(2) \textbf{hypernymy organization} (i.e., organizing extracted term pairs into a taxonomy). 
The first phase outputs a collection of candidate hypernymy relations, based on which a dense and noisy hypernym graph is built.
Then, the second phase inducts a tree-structured taxonomy from the hypernym graph using graph-based methods. 
These methods include maximum spanning tree (MST) \cite{navigli2011graph,anh2014taxonomy,bansal2014structured,zhang2016learning}, minimum-cost flow (MCF) \cite{gupta2017taxonomy}, and other graph pruning heuristics \cite{kozareva2010semi,velardi2013ontolearn,faralli2015large,panchenko2016taxi}.

%The second phase, hypernymy organization, is usually based on the output of the first phase.
% There are various approaches \cite{kozareva2010semi,anh2014taxonomy,velardi2013ontolearn,bansal2014structured,zhang2016learning,panchenko2016taxi,gupta2017taxonomy} to automatic taxonomy induction. 
% However, most (if not all) of them still regard the two phases as two \emph{separate} steps and perform them sequentially.
% In the first phase, hypernyms are detected: either hypernym pairs are found or the weights of every term pair being hypernym are estimated.
% In this way, a dense, noisy hypernym graph consisting of term pairs is generated. 
%Specifically, one taxonomy is constructed from the noisy hypernym graph extracted in the first phase.  
%and other graph pruning approachesare used to ensure that the final output of taxonomy induction is a tree-structured hierarchy.


\nop{ % Yuning
As pointed out in \citet{gupta2017taxonomy,camacho2017we}, approaches towards automatic taxonomy induction are generally composed of two phases: \textbf{extraction of hypernymy relations} (i.e., ``is-a'' relations between term pairs, such as (beef, meat)) and \textbf{hypernymy organization of term pairs into a taxonomy}.
}
% (i.e., pruning the noisy hypernym graph extracted in the first phase into a coherent tree-structured hierarchy)
\begin{figure*}[ht]
    \centering
    \includegraphics[width=16cm, height=2.2cm]{fig/dog}
    % \caption{A toy example that shows how a taxonomy is constructed in our framework:  staring from an empty taxonomy, the terms in the input vocabulary are added to the taxonomy one at a time. The agent needs to learn which term to select and where to attach it.}
     \caption{An illustrative example showing the process of taxonomy induction. 
The input vocabulary $V_0$ is \{\mquote{working dog}, \mquote{pinscher}, \mquote{shepherd dog}, ...\}, and the initial taxonomy $T_{0}$ is empty. 
%The size of the vocabulary $|V_0|$ is 8.
%At the beginning of the episode, there is no term on the taxonomy.
We use a virtual \mquote{root} node to represent $T_{0}$ at $t=0$. 
%The next figure shows the taxonomy at time step $t=5$, when there are 5 terms on the taxonomy and  3 ($|V_0| - t$) terms left to attach: $V_t$ = \{shepherd dog, collie, affenpinscher\}.
At time $t=5$, there are 5 terms on the taxonomy $T_{5}$ and 3 terms left to be attached: $V_t$ = \{\mquote{shepherd dog}, \mquote{collie}, \mquote{affenpinscher}\}.
Suppose the term \mquote{affenpinscher} is selected and put under \mquote{pinscher}, then the remaining vocabulary $V_{t+1}$ at next time step becomes \{\mquote{shepherd dog}, \mquote{collie}\}.
%Assume the term pair (pinscher, affenpinscher) is selected, the remaining vocabulary $V_{t+1}$ at next time step then becomes \{shepherd dog, collie\}.
Finally, after $|V_0|$ time steps, all the terms are attached to the taxonomy and $V_{|V_0|} = V_{8} = \{ \}$.
%A full taxonomy consisting of all terms in the input vocabulary is constructed from scratch.
A full taxonomy is then constructed from scratch.
}
    \label{fig:toy}
    \vspace*{-.4cm}
\end{figure*}


% \nop{ % Yuning
% % Many methods are proposed in the prior literature which focus on extracting hypernyms with high quality but do not organize them further into a tree-like hierarchy.
% % The main categories of hypernymy detection methods include pattern-based and distributional approaches.
% % Pattern-based approaches use lexico-syntactic patterns to capture hypernym relations.
% % Such patterns can be either manually designed \cite{hearst1992automatic,kozareva2010semi} or learned from corpora \cite{snow2005learning,bansal2014structured}.
% % % Pattern-based approaches generally achieve high precision but suffer from low recall.
% % % In addition, it requires that the hypernyms appear together to be detected.
% % Distributional approaches utilize the distributional representations of terms/term pairs for hypernymy detection.
% % Some of them \cite{weeds2004characterising,roller2014inclusive,chang2017unsupervised} are based on the Distributional Inclusion Hypothesis \cite{geffet2005distributional}, which assumes that a hypernym has broader contexts than its hyponyms.
% % Others \cite{fu2014learning,yu2015learning,tuan2016learning,NIPS2017_7213} learn term embeddings and detect hypernyms in a supervised fashion.
% % % Contextual information between term pairs is also leveraged in recent works \cite{tuan2016learning, shwartz2016improving}.
% The first phase, largely referred as hypernymy detection, has been well studied.
% The second phase, hypernymy organization, is usually based on the output of the first phase.
% % There are various approaches \cite{kozareva2010semi,anh2014taxonomy,velardi2013ontolearn,bansal2014structured,zhang2016learning,panchenko2016taxi,gupta2017taxonomy} to automatic taxonomy induction. 
% % However, most (if not all) of them still regard the two phases as two \emph{separate} steps and perform them sequentially.
% % In the first phase, hypernyms are detected: either hypernym pairs are found or the weights of every term pair being hypernym are estimated.
% % In this way, a dense, noisy hypernym graph consisting of term pairs is generated. 
% Specifically, one taxonomy is constructed from the noisy hypernym graph extracted in the first phase.  
% Maximum spanning tree (MST) \cite{navigli2011graph,anh2014taxonomy,bansal2014structured,zhang2016learning}, minimum-cost flow (MCF) \cite{gupta2017taxonomy}, and other graph pruning approaches \cite{kozareva2010semi,velardi2013ontolearn,faralli2015large,panchenko2016taxi} are used to ensure that the final output of taxonomy induction is a tree-structured hierarchy.
% }

%% JS
These two-phase approaches have several limitations: most of them \cite{kozareva2010semi,anh2014taxonomy,panchenko2016taxi,gupta2017taxonomy} ignore the overall taxonomy structure when estimating the probability that a term pair holds the hypernymy relation.
They treat each term pair equally and estimate the probability of different term pairs independently.
In consequence, possibly wrong estimations cannot be rectified based on the results of hypernymy organization, which causes the error propagation problem. 
Some works \cite{bansal2014structured,zhang2016learning} do explore the taxonomy space by regarding the induction of taxonomy structure as inferring the conditional distribution of edges. 
In other words, they use the product of edge probabilities to represent the taxonomy quality.
However, edges are still treated equally, while in reality, they contribute to the taxonomy differently.
For example, a high up edge is likely to be more important than a bottom-out edge because it has much more influence on its descendants.

% \nop{ % Yuning
% Traditional two-phase approaches have several limitations: most \cite{kozareva2010semi,anh2014taxonomy,panchenko2016taxi,gupta2017taxonomy} of them ignore the overall taxonomy structure when estimating the probability of hypernymy relation between a term pair.
% Each term pair is treated equally and the estimations of different term pairs are performed independently.
% In consequence, the estimations cannot be rectified based on the results of hypernymy organization and the errors in the first phase would inevitably propagate to the second phase. 
% Some \cite{bansal2014structured,zhang2016learning} do explore the taxonomy space by regarding the induction of taxonomy structure as inferring the conditional distribution of edges, i.e., using the sum of edge scores to represent the quality of a taxonomy.
% However, edges are still treated equally, while contributing to the taxonomy differently.
% For example, a high up edge is likely to be more important than a bottom-out edge because it has much more influence on its descendants.
% }

%% JS
To address these issues, we propose to jointly conduct hypernymy detection and hypernymy organization by learning term pair representations and constructing the taxonomy simultaneously. 
The feedback during hypernymy organization is propagated back to the hypernymy detection phase, based on which the term pair representations are rectified.
As a result, the learned representations encode not only the local information between a term pair but also the global taxonomy structure.
Moreover, we optimize a holistic metric in a joint learning scheme beyond pairwise or local objectives. 
The probability of a full taxonomy is no longer a simple aggregated probability of its edges.
Instead, we assess an edge based on how much it can contribute to the whole quality of the taxonomy.

%% JS
Since it is infeasible to estimate the quality of all possible taxonomies, we propose a novel reinforcement learning (RL) framework to combine the two phases.
Specifically, we train an RL agent that learns how to select terms from a vocabulary and then attach them one at a time to an empty taxonomy until a whole taxonomy is constructed.
We perform two sets of experiments to demonstrate the superiority of our framework.
First, we compare the performance of our RL framework with two-phase approaches, and show that our framework outperforms them significantly, even when the same term pair representation is used as input.
Secondly, we use the same noisy hypernym graph as the input of our framework and baselines, and show that our framework is better at hypernymy organization by leveraging the global taxonomy structure.


\nop{ % Yuning
Since it is infeasible to estimate the quality of all possible taxonomies, we design a reinforcement learning (RL) framework for the combination of the two phases.
Specifically, we train an RL agent that learns how to select terms from a vocabulary and then attach them one at a time to an empty taxonomy until a whole taxonomy is constructed.
We perform two sets of experiments to demonstrate the superiority of our framework.
First, we compare the performance of our joint learning framework with two-phase approaches and show that our framework outperforms two-phase approaches significantly, even when the same term pair representation is used as input.
Secondly, we use the same noisy hypernym graph as the input of our framework and baselines and show that our framework is better at hypernymy organization by considering the global structure.
}

In summary, we have made the following contributions:
(1) We propose the first end-to-end deep reinforcement learning framework that combines the phases of hypernymy detection and hypernymy organization in a more unified way.
% (2) We bridge the gap between (pure) hypernymy detection methods and taxonomy induction methods. Models and features that are capable of capturing (non-edge) hypernymy relations can be easily incorporated into our framework and help with taxonomy induction. 
(2) We show that the error propagation between the two phases is effectively reduced and global taxonomy structure is better captured using this novel framework. 
(3) We compare our framework with existing state-of-the-art models on datasets in different domains and show that our methodology exhibits superior performance.

The rest of the paper is organized as follows.
We formalize the problem in Section \ref{definition}.
We introduce the hypernymy detection model in Section \ref{hyper}.
We present our RL framework in Section \ref{rl}. 
We discuss experimental setups and results in Section \ref{exp}, 
and conduct analysis in Section \ref{casestudy}. 
We review related work in Section \ref{related-work},
and conclude the paper in Section \ref{conclusion}.


==> 2-problem.tex <==
%!TEX root = acl18-RL-tree.tex
% UTF-8 encoding

\section{Problem Formulation} \label{definition}

We define a taxonomy $T$ as a data model that represents a set of terms $V$ and a set of relations $R$ between these terms \cite{yang2009metric}.
%Therefore, $T$ can be also written as $T(V,R)$.
Given an input vocabulary $V_{0}$, a \emph{full taxonomy} is a tree-structured hierarchy that contains all the terms in $V_{0}$, and a \emph{partial taxonomy} is a hierarchy containing only a subset of terms in $V_{0}$. 
In our end-to-end learning framework, we aim to learn a model such that given an input vocabulary $V_{0}$ and an empty taxonomy $T_{0}$, it can construct a full taxonomy $T$ by adding terms from $V_{0}$ onto $T_0$ one at a time.
An illustrative example is shown in Fig.~\ref{fig:toy}.



\nop{ % Yuning
We assume that the vocabulary needed for taxonomy induction is provided as input.
Given an input vocabulary $V$ and an empty taxonomy $T$, the goal of our task is to learn the principles of attaching terms in $V$ to the taxonomy $T$ one at a time.
We formulate the problem as follows: at each time step, we estimate the probabilities of edges between all possible term pairs consisting of one term in $V$ and one on the current taxonomy $T$.
The estimation is performed simultaneously with the learning of term pair representations, and the final selection of term pair at one time step is sampled by the probability distribution of term pairs at that time step.
After a term pair $(x_1, x_2)$ is selected, we remove term $x_1$ (which is not on the current taxonomy) from the vocabulary $V$ and attach it to $T$ by adding an edge between $x_1$ and $x_2$.
The steps above are repeated until a taxonomy is finally constructed from scratch.
A concrete example is shown in Fig.~\ref{fig:toy}.
}



% A concrete example is shown in Figure \ref{fig:toy}.
% % A concrete example illustrating how a taxonomy is constructed in our framework can be found in Figure \ref{fig:toy}.
% In this example, the input vocabulary $V_0$ is \{working dog, pinscher, shepherd dog, ...\}.
% The size of the vocabulary $|V_0|$ is 8.
% At the beginning of the episode, there is no term on the taxonomy.
% We use a virtual root node to represent an empty taxonomy for convenience.
% The next figure shows the taxonomy at time step $t=5$, when there are 5 terms on the taxonomy and  3 ($|V_0| - t$) terms left to attach: $V_t$ = \{shepherd dog, collie, affenpinscher\}.
% Assume the term pair (pinscher, affenpinscher) is selected, the remaining vocabulary $V_{t+1}$ at next time step then becomes \{shepherd dog, collie\}.
% After $|V_0|$ time steps, all the terms are attached to the taxonomy and $V_{|V_0|} = V_8 = \{ \}$.
% A full taxonomy consisting of terms in the input vocabulary is  constructed from scratch.





==> 3-hypernym-model.tex <==
%!TEX root = acl18-RL-tree.tex
% UTF-8 encoding

\section{Hypernymy Detection Model} \label{hyper}

A good representation of hypernymy relations is critical to automatic taxonomy induction. 
We follow HypeNET \cite{shwartz2016improving}, a state-of-the-art hypernymy detection model, to learn hypernymy relation representations.
HypeNET only leverages path-based and distributional information, and we extend it by incorporating more features that are proved effective for hypernymy detection in previous works \cite{bansal2014structured,gupta2017taxonomy}.
Such combination of information from different sources can better represent the semantic relation between a term pair and is crucial to our task.
% Following we give detailed descriptions for each type of features.

\nop{ % Yuning
One of the keys to constructing a taxonomy with high quality is to have a good representation of its hypernyms.
% \footnote{A newer version of HypeNET. Available at https://github.com/vered1986/HypeNET}
We follow HypeNET \cite{shwartz2016improving}, one of the state-of-the-art models for classifying semantic relations, to learn hypernym representations.
In addition to the path-based and distributional information that HypeNET used, we further combine features that were shown to be effective in previous works \cite{bansal2014structured,gupta2017taxonomy}.
% on one hand, it leverages path-based information, which is extracted from the shortest dependency paths between term pairs and encoded using a Long short-term memory (LSTM).
% On the other hand, it uses distributional information of each term, which is obtained by pre-trained word embeddings.
}

\textbf{Path-based Information.}
We extract the shortest dependency paths between each term pair from the text corpora.
%For path-based information, the shortest dependency paths between term pairs are extracted from text corpora. 
Each dependency path is represented as a sequence of edges that goes from term $x$ to term $y$ in the dependency tree,
and each edge consists of the word lemma, the part-of-speech tag, the dependency label and the edge direction between two contiguous words.
The edge is represented by the concatenation of embeddings of its four components:
\begin{equation*}
\textbf{V}_{e} = [\textbf{V}_{l},, \textbf{V}_{\text{pos}}, \textbf{V}_{\text{dep}}, \textbf{V}_{\text{dir}}].
\end{equation*}
%Instead of treating the entire dependency path as a single feature, the sequence of dependency edges $\textbf{V}_{e_1}, \textbf{V}_{e_2}, ..., \textbf{V}_{e_k}$ is encoded using an LSTM so that the model learns to focus on parts of the path that are more informative for term pair representation learning while ignoring others.
Instead of treating the entire dependency path as a single feature, we encode the sequence of dependency edges $\textbf{V}_{e_1}, \textbf{V}_{e_2}, ..., \textbf{V}_{e_k}$ using an LSTM so that the model can focus on learning from parts of the path that are more informative while ignoring others.
We denote the final output of the LSTM for path $p$ as $\textbf{O}_p$, and use $\mathcal{P}(x, y)$ to represent the set of all dependency paths between term pair $(x, y)$.
%We denote the dependency paths between term pair $(x, y)$ as $\mathcal{P}(x, y)$.
A single vector representation of the term pair $(x, y)$ is then computed as $\textbf{P}_{\mathcal{P}(x,y)}$, the weighted average of all its path representations by applying an average pooling:
\begin{equation*}
\textbf{P}_{\mathcal{P}(x,y)} = \frac{\sum_{p \in \mathcal{P}(x, y)} c_{(x,y)}(p) \cdot \textbf{O}_p}{\sum_{p \in \mathcal{P}(x, y)} c_{(x,y)}(p) },
\end{equation*}
where $c_{(x,y)}(p)$ denotes the frequency of path $p$ in $\mathcal{P}(x, y)$.
For those term pairs without dependency paths, we use a randomly initialized \emph{empty path} to represent them as in HypeNET. 

\textbf{Distributional Information.}
The previous path-based features are only applicable when two terms co-occur in a sentence. 
In our experiments, however, we found that only about 17\% of term pairs have sentence-level co-occurrences.\footnote{In comparison, more than 70\% of term pairs have sentence-level co-occurrences in BLESS \cite{baroni2011we}, a standard hypernymy detection dataset.}
To alleviate the sparsity problem, we concatenate the path representation $\textbf{P}_{\mathcal{P}(x,y)}$ with the word embeddings of $x$ and $y$, which capture the distributional information of two terms.


%For distributional information, the word embeddings of $x$ and $y$ are concatenated to the path representation $\textbf{P}_{\mathcal{P}(x,y)}$, which further capture the relation between a term pair.
%Note that such combination of information from multiple sources is crucial to our task because the co-occurrences of term pairs in taxonomy induction are much more sparse than in the standard hypernymy detection datasets (e.g., BLESS \cite{baroni2011we})
%\footnote{In our experiments, the ratio of co-occurrence of term pairs is below 10\% on average. In contrast, the ratio is more than 70\% in BLESS and 100\% in relation extraction/classification datasets.}.
% which makes taxonomy induction much harder than the binary classification of hypernym pairs.
%In consequence, it is unlikely that one can find relevant sentences for every term pair, let along extracting dependency paths between them.

\textbf{Surface Features.}
In practice, even the embeddings of many terms are missing because the terms in the input vocabulary may be phrases or entities,
which are not usually covered by the pre-trained word embeddings.
To tackle this issue, 
we utilize several surface features described in previous studies \cite{yang2009metric, bansal2014structured, zhang2016learning}.
Specifically, we employ \emph{Capitalization}, \emph{Ends with}, \emph{Contains}, \emph{Suffix match}, \emph{Longest common substring} and \emph{Length difference}.
These features are effective for detecting hypernyms solely based on the term pairs.



\textbf{Frequency and Generality Features.}
Another feature source that we employ is the hypernym candidates from TAXI\footnote{http://tudarmstadt-lt.github.io/taxi/} \cite{panchenko2016taxi}.
These hypernym candidates are extracted by lexico-syntactic patterns and contain noise.
Since only term pairs and their raw frequencies are available from this resource, we cannot recover the patterns of dependency paths based on it.
We hence design two features that are similar to those used in \citet{panchenko2016taxi,gupta2017taxonomy}.
\footnote{Since the features require additional resource, we wouldn't include them unless otherwise specified.}
%Due to the same reason above, we reuse the hypernym candidates from TAXI\footnote{Available at http://tudarmstadt-lt.github.io/taxi/. Since it used additional resources, we wouldn't include frequency features unless otherwise specified.} \cite{panchenko2016taxi} in addition to the path-based and distributional information as in HypeNET.
%Since only term pairs and their raw frequencies are available from this resource, it is impossible to recover patterns or dependency paths.
%We hence design two frequency features that are similar to those used in \citet{panchenko2016taxi,gupta2017taxonomy}.
\begin{itemize}[leftmargin=*]
  \item \emph{Normalized Frequency Diff.} 
  % This feature is an asymmetric hypernymy score based on the frequency of term pairs.
  For a hyponym-hypernym pair $(x_i, x_j)$ where $x_i$ is the hyponym and $x_j$ is the hypernym, its normalized frequency is defined as $\text{freq}_n(x_i, x_j) = \frac{\text{freq}(x_i, x_j)}{\max_k \text{freq}(x_i, x_k)}$, where $\text{freq}(x_i, x_j)$ denotes the raw frequency of $(x_i, x_j)$.
  The final feature score is defined as $\text{freq}_n(x_i, x_j) - \text{freq}_n(x_j, x_i)$, which down-ranks synonyms and co-hyponyms.
  Intuitively, a higher score indicates a higher probability that the given term pair holds the hypernymy relation. 
  \item \emph{Generality Diff.} 
  The generality $g(x)$ of a term $x$ is defined as the logarithm of the number of its distinct hyponyms, i.e., $g(x) = log(1 + |\textbf{hypo}|)$, where for any $hypo \in \textbf{hypo}$, $(hypo, x)$ is a hypernym candidate.
  A high $g(x)$ of the term $x$  implies that $x$ is general since it has many distinct hyponyms.
  The generality of a term pair is defined as the difference in generality between $x_j$ and $x_i$: $g(x_j) - g(x_i)$.
  This feature would promote term pairs with the right level of generality and penalize term pairs that are either too general or too specific.
\end{itemize}

The surface, frequency, and generality features are binned and their embeddings are concatenated as a part of the term pair representation.
In summary, the final term pair representation $\textbf{R}_{xy}$ has the following form:
\begin{equation*}
\textbf{R}_{xy} = [\textbf{P}_{\mathcal{P}(x,y)}, \textbf{V}_{w_x}, \textbf{V}_{w_y}, \textbf{V}_{F(x,y)}],
\end{equation*}
where $\textbf{P}_{\mathcal{P}(x,y)}$, $\textbf{V}_{w_x}$, $\textbf{V}_{w_y}$, $\textbf{V}_{F(x,y)}$ denote the path representation, the word embedding of $x$ and $y$, and the feature embeddings, respectively.

Finally, we would like to emphasize that although we use HypeNET to learn term pair representations, any other relation extraction models, such as \citet{zhang2017position,lin2016neural}, can be easily incorporated into our framework, as long as they can encode the relation between a term pair into a vector representation. 
%capture the relation between term pairs and produce a vector representation for each of them.
% However, the exploration towards this direction is orthogonal to our work and we wouldn't discuss the advantages and disadvantages of different relation extraction models for hypernymy detection. 

